Deterministic Near-Linear Time Minimum Cut in Weighted Graphs

In 1996, Karger [Kar96] gave a startling randomized algorithm that finds a minimum-cut in a (weighted) graph in time $O(m\log^3n)$ which he termed near-linear time meaning linear (in the size of the input) times a polylogarthmic factor. In this paper, we give the first deterministic algorithm which runs in near-linear time for weighted graphs. Previously, the breakthrough results of Kawarabayashi and Thorup [KT19] gave a near-linear time algorithm for simple graphs. The main technique here is a clustering procedure that perfectly preserves minimum cuts. Recently, Li [Li21] gave an $m^{1+o(1)}$ deterministic minimum-cut algorithm for weighted graphs; this form of running time has been termed "almost-linear''. Li uses almost-linear time deterministic expander decompositions which do not perfectly preserve minimum cuts, but he can use these clusterings to, in a sense, "derandomize'' the methods of Karger. In terms of techniques, we provide a structural theorem that says there exists a sparse clustering that preserves minimum cuts in a weighted graph with $o(1)$ error. In addition, we construct it deterministically in near linear time. This was done exactly for simple graphs in [KT19, HRW20] and with polylogarithmic error for weighted graphs in [Li21]. Extending the techniques in [KT19, HRW20] to weighted graphs presents significant challenges, and moreover, the algorithm can only polylogarithmically approximately preserve minimum cuts. A remaining challenge is to reduce the polylogarithmic-approximate clusterings to $1+o(1/\log n)$-approximate so that they can be applied recursively as in [Li21] over $O(\log n)$ many levels. This is an additional challenge that requires building on properties of tree-packings in the presence of a wide range of edge weights to, for example, find sources for local flow computations which identify minimum cuts that cross clusters.

==> sampling.tex <==
\section{Sampling}\label{sec:sampling}


In this section, we use techniques from \cite{Li21} to build a sparse
graph that approximates all the minimum cuts in a graph $G$ given
our decompositions from the previous sections. 

We begin with some definitions that parallel those in \cite{Li21}. In
particular, the decomposition sequence below is essentially the same
as Li's decomposition sequence except it uses our partitioning scheme
rather than expander decompositions.

\begin{definition}
  Let $\alpha \ge 0$.
  A set $S \subset V$ is $(\alpha,s_0)$ uncrossable with a set $A$ if
  \begin{enumerate}
  \item
    $w(S\cap A, S \cap \overline{A} ) \leq \alpha w(S\cap A, \overline{S} \cap A)$ and $\vol(A \cap S) \leq s_0$, or 
  \item
    $w(A \setminus S,  \overline{A} \setminus S) \leq \alpha w(S\cap A, \overline{S} \cap A)$ and $\vol(A \setminus S) \leq s_0$.      
  \end{enumerate}

  The set $A$ is an {\em uncrossing} of $S$ with respect to $A \cap S$, if the first case holds, and with respect to $A \setminus S$ if the second case holds.

\end{definition}

Note that if $S \cap A = \emptyset$ then $S$ is $(\alpha, s)$ uncrossable with $A$ for any $\alpha$ and any $s\ge 0$ as condition 1 holds trivially.
If $S \cap A = A$, i.e. $A \setminus S = \emptyset$,
%$S \cap A \subseteq S$, 
then $S$ is $(\alpha, s)$ uncrossable with $A$ for any $\alpha$ and any $s\ge 0$ as condition 2 holds trivially.


\begin{definition}

  Let $\alpha \ge 0$.
  Given a graph $G=(V,E)$, assume $V$ is partitioned into vertex sets $\{A_1,\ldots,A_k\}$. Then $\{A_1,\ldots,A_k\}$  is
  $(\alpha,s_0)$-uncrossable if for any $2$-approximate minimum
  cut $S\subseteq V$ of $G$, there is a partition $\mathcal P$ of the
  set $\{A_1,A_2,\ldots,A_k\}$ such that $S$
  is
  $(\alpha,s_0)$-uncrossable with respect to $\cup_{j = 1}^\ell A_{i_j}$ for each element
  $P=\{A_{i_1},\ldots,A_{i_\ell}\}\in\mathcal P$.

\end{definition}



\begin{definition}
  
  An {$(\epsilon,s_0)$}-decomposition sequence of a graph $G = (V,E)$
  is a $(\epsilon,s_0)$-partition of $G$, $\{A_1,\ldots,A_k\}$, and an
  $(\epsilon,s_0)$-decomposition sequence of $G' = (V',E')$ where $V'$ contains
  a vertex for each $A_i$, and $E' = \{(A_i,A_k) : (u,v) \in E, u \in
  A_i, v \in A_k\}$ (there may be parallel edges).  

\end{definition}
\mh{What is a $(\epsilon,s_0)$-partition of $G$? Do you mean it is a partition that is $(1+\epsilon, s_0)$-uncrossable?}
\mh{we should say more clearly that we do not recursively decompose graphs with volume $< s_0$.}

Note that a graph $G=(V,E)$ of volume $s_0$ forms by itself a trivial
decomposition sequence.

We reframe the decomposition using the notation from \cite{Li21}.

For a graph $G$ and an $(\epsilon,s_0)$-decomposition, $G^{0}$ denotes
the original graph, and $G^{(i)}$ denotes the graph obtained after $i$
levels of recursion and ${(A^{i}_1, \ldots, A^{i}_{k_i}})$ denotes the
$(\epsilon,s_0)$ partition of graph $G^{(i)}$. Note, for example, that
$G^{i+1}$ has a vertex for each group of vertices in $A^{i}_j$ and
that the edges in $G^{(i+1)}$ correspond to edges in $G^{(i)}$. In the
context of this correspondence, we have $E(G^{0}) \supseteq E(G^{1})
\supseteq \cdots$.

As from \cite{Li21}, for a cut $S$ in $G = (V,E)$ and an
$(\epsilon,s_0)$-decomposition, let $S^{0}$ is $S$, and $S^{i}$
contains vertices of $G^{i+1}$ specified below.  For a vertex $v_j$ corresponding to
$A^{i}_j$, Li \cite{Li21} defines $D_{j}^i = A_{j}^i / S^{i}$\mh{setminus?} if $v_j
\in S^{i+1}$ and $D_{j}^i = A_{j}^i \cup S^{i}$ otherwise.  Note,
these definitions are valid for an arbitrary assignment of vertices to
$S^{i}$.


We now specify $S^{i+1}$ as follows. Consider the
$(\epsilon,s_0)$-uncrossable sets $\{A_1^i,\ldots,A^i_{k_i}\}$
and the partition ${\cal P}$ for $S^{i}$.  The uncrossing of $S^{i}$
for each part entirely contains or entirely does not contain each
$A_j^{i}$ and $v_j$ is included in $S^{i+1}$ accordingly.

We denote this sequence for $S$
as $\{S^i\}$ and
consider $D_i^j$ to be defined with respect to the $\{S^i\}$
and let $L$ be the number of levels in the sequence.

Let us define $\nabla_G(S)$ to consist of all edges of $G$ with exactly one endpoint in $S$.
We then have Lemma 3.3 in \cite{Li21} restated here.

\begin{lemma}

  For any decomposition sequence $\{S_i \}$ of $S$,

  $$\nabla_G S \subseteq \cup_{i,j} \nabla_{G^{i}} D_j^i.$$

\end{lemma}
We have the following lemma which is analagous to the Lemma 3.4 in \cite{Li21}.

\begin{lemma}
\label{lem:dij-vol-bound}

  If $\epsilon < .01/L$, 

  $$\sum_{i,j} w(\partial_{G^i} D^i_j) \leq 2 L s_0$$
  
  
\end{lemma}

{\bf Proof:}

From the definition of $(\epsilon,s_0)$-uncrossable and
$\epsilon \leq 1/L$, we have $ w(\nabla S^{i}) \leq (1+\epsilon)^i
w(\nabla S)$ since each $S^i$ can be uncrossed into $S^{i+1}$ as the cut
size is smaller than $e^{.1} w(\nabla S)$.\mh{where does that come from and what does it say?}

By the definition of uncrossable, 
each $D_j^i$ consists of at most $s_0$ volume in $G^i$, and thus the
total volume is $\nabla D_i^k$ is $s_0 L$.
\mh{Do you mean $\vol(\cup_{j} D_j^L) \le s_0 (1+\epsilon)^L w(\nabla S)=
s_0 e^{0.01} w(\nabla S)$?}

It follows that 
 $$\sum_{i,j} w(\partial_{G^i} D^i_j) \leq  2 s_0 L.$$
\qed


As in \cite{Li21}, we define the ``pullback'', $\overline{v}$, of a
vertex $v \in G^{i}$ as the set of vertices in $V$ that were
contracted to make $v$ through the series of contractions.  And the
pullback $\overline{D}_j^i$ as the union of the pullbacks of the
vertices in $G^i$ that comprise $D_j^i$.  By construction, $S$
can be constructed using the $D_j^i$ corresponding to the sequence $\{S^i\}$
with unions and differences and can write

$$\mathbbm{1}_S = \sum_{i,j} \pm \mathbbm{1}_{\overline{D}^i_j} = \sum_{i,j} \sum_{\overline{v} \in \overline{D}^i_j} \pm \mathbbm{1}_{\overline{v}},$$

where the $\pm$ corresponds to differences or unions and

$$w(\nabla_G S) = \mathbbm{1}_S^T L_S \mathbbm{1}_{S} = \sum_{i,j,k,l} \pm
\mathbbm{1}_{\overline{D}^i_j} L_{S} \pm \mathbbm{1}_{\overline{D}^k_l}
L_{S}.$$

This is exactly equation $9$ in \cite{Li21} and given
lemma~\ref{lem:dij-vol-bound} we can conclude that there are at most
$s_0^2L^2$ terms in the summation for $\nabla_G(G)$.

Thus, if one can create a graph, $H$, on $V$ where the weights of all
pairs of the sets $\overline{D}_j^i$ are appropximated to within an
additive factor of $\epsilon \lambda /(s_0^2 L^2)$ then graph will
also approximate the value of $w(\nabla_G(S))$ to with an additive
$\epsilon \lambda$.

The derandomized sampling procedure in section~{3.2.1} in \cite{Li21}
allows us to do so with a number of edges and running time that is
$\tilde{O}(m \epsilon^2 L^4 s_0^4)$.








==> techniques.tex <==
%\section{Techniques}

We discuss in more detail some of the techniques that
we build upon along with a description of our contributions.

A classical result of Nash and Williams \cite{nash1961edge} showed that any graph
$G$ with minimum cut $\lambda$ contains a packing of $\lambda$
arborescences (directed trees) in the directed graph where each edge
in $G$ is replaced by an edge in each direction. Gabow \cite{gabo1995matroid}
provided a relatively efficient $\tilde{O}(\lambda m)$ algorithm that
produced the packing. There are randomized approximation algorithms that
produce fractional and approximate packings as well
\cite{plotkin1995fast}.

As noted previously, in 1996, Karger's famous paper \cite{KargerStoc}
gave an $O(m \log^3 n)$ randomized min-cut algorithm that takes a graph $G$
and produces a weighted graph with $O(n\log n)$ edges where the
minimum cuts are preserved to within a $(1+\epsilon)$
factor.\footnote{This work is inspired by a sequence of previous
papers on randomized approaches that remained far from near linear
time. \cite{karger1996new,benczur1996approximatingbenczur2015randomized}.}
Then Karger builds a tree packing using \cite{gabo1995matroid} in
that weighted graph that consists of $O(\log n)$ trees.  In such a
tree packing, there must be a tree which intersects the minimum-cut at
most twice, and Karger provides an efficient dynamic programming
algorithm that given that tree produces a minimum cut.

Karger produces the sparse graph by sampling edges inversely to their
``strength'', a measure of the connectivity of the endpoints, in a
manner that preserves all small cuts and yields a sparse
graph. Specifically, the sampling introduces an edge of weight $1/p$ if
an edge is sampled with probability $p$, which preserves the edge on
expectation, and sampling by strength preserves all cuts with high
probability, which can be argued using the bounds on the number of
minimum-cuts and near minimum-cuts as follows from
\cite{karger1996new}. This sampling procedure was very much
randomized and an efficient deterministic construction has remained
elusive.
%
We note that Karger's algorithm works naturally for weighted graphs.

In a breakthrough in 2015, Thorup and Kawarabayashi \cite{KawarabayashiT19} gave a
deterministic algorithm for simple graphs with running time
$\tilde{O}(m)$. This was improved 
%by a subset of the current authors
to run in time $O(m \log^2n \log\log n)$ for simple graphs
\cite{DBLP:journals/siamcomp/HenzingerRW20}.\footnote{While the running time is better than Karger's
randomized algorithm, subsequent work has provided an $O(m\log^2n)$
time randomized algorithm for minimum cut in simple graphs \cite{gawrychowski2020minimum}.}

The idea in those papers is to produce a sparse graph by producing a
hierarchical clustering. At each level, a set of clusters is produced
such that no non-trivial\footnote{A trivial cut consists of just one
vertex.} minimum-cut separates any cluster and has few intercluster
edges. Thus, collapsing the graph and recursing ensures that all
non-trivial minimum cuts are preserved. The collapsing can be repeated until the
graph has $m' = \tilde{O}(m/\delta)$ edges where $\delta$ is the minimum degree, and then simply run Gabow's
algorithm \cite{Gabow} to find a minimum cut in $\tilde{O}(\lambda\cdot m/\delta)=\tilde{O}(m)$
time. 

An example is useful here. First, note that a simple cycle is ``easy''
in the sense it is sparse and one can simply run Gabow \cite{gabo1995matroid} in
linear time.  Replacing each vertex with a clique on $\delta$ vertices
and connecting  the corresponding vertices along the cycle produces a
``dense'' graph with minimum degree and cut size $\approx\delta$.  The algorithms in
\cite{KawarabayashiT19,DBLP:journals/siamcomp/HenzingerRW20} produce a
final graph whose clusters \mh{nodes?} are the cliques, which will not be split by
any minimum cut.  The number of edges, including parallel edges, in
the collapsed graph is $O(m/\delta)$ and this graph contains all non-trivial
minimum cuts in the original graph.  Inspired by this example, we say a vertex clustering is  \emph{non-crossed} if there exists a minimum cut that does not cut any of the clusters.

To proceed it is useful to provide a little more detail.  The
algorithms of
\cite{KawarabayashiT19,DBLP:journals/siamcomp/HenzingerRW20} produce
the non-crossed clusterings incrementally. That is, their
algorithm begins with a partition where any minimum cut only overlaps (i.e., crosses)
any piece by some volume $s$, which is initially $m/2$, and then proceeds to iteratively refine that
clustering, in each iteration decreasing $s$ by a factor of $2$.  Once $s$ is
smaller than $\Theta(\delta)$ they clean up the resulting partition to
obtain the property that a non-trivial minimum cut does not cross any of the
resulting clusters at all. This last step of obtaining perfectly
non-crossing clusterings relies crucially on the property of simple
graphs, such as the fact that any minimum cut in a simple graph consists
of either a single vertex or at least $\delta$ vertices.


Moreover, the recursive techniques face substantial issues for weighted graphs
in terms of complexity. The refinement process in
\cite{DBLP:journals/siamcomp/HenzingerRW20} performs local flow
computations where the progress is proportional to the total weight of the 
edges that are touched.  In simple graphs, the weight and the number of
edges are the same and thus the total work is near-linear in the number
of edges.  For weighted graphs, the number of edges and the total
weight differ and we, thus, need to devise new algorithms for
the refinement process.  Another issue in the refinement process is
the allocation of sources for the local flows which also is more
complex as weighted graphs do not ``expand'' with respect to weights
as fast as simple graphs expand with respect to degrees. E.g., a
degree $\delta$ simple graph has $\delta$-neighbors, where a vertex of
weighted degree of $\delta$ may have a single neighbor.

This expansion issue creates an even bigger obstruction for going
from ``almost'' non-crossed as defined by $s$ to completely
non-crossing.  This barrier remains and we do not produce a clustering
such that every cluster is non-crossed in this work.

Fortunately, Li \cite{Li21} provides an ingenious approach for utilizing
approximately non-crossing clusterings to derandomize the sampling
approach of Karger \cite{karger1996new}. He first shows how to use expander
decompositions to produce approximately non-crossing
clusterings\footnote{The technical definitions of approximately
non-crossing are a bit different than those in \cite{KawarabayashiT19,DBLP:journals/siamcomp/HenzingerRW20} and here,
but are similar in consequence.}, the deterministic constructions of
which take $m^{1+o(\epsilon)}$ time. He introduced another measure of
non-crossing of cuts for the partition in addition to the volume $s$ of
overlap. In particular, his clusterings ensuring that making a cut
consistent with a clustering would only increase its size by an
$n^{o(1)}$ factor. This is what he calls \emph{uncrossing} a cut. He could then produce a hierarchical clustering
where every minimum cut is well approximated by an arithmetic
expression using a small linear number of the clusters in the hierarchy.

He argued further that sampling a subset of edges that approximately
preserves the boundary size of the near linear number of clusters
would then preserve approximately the minimum cuts as well.  This
contrasts with Karger's sampling which argued about an exponential
number of cuts.  The linear number of cuts allows one to derandomize
the selection of edges as one can explicitly measure each of the cuts
as one chooses edges to include in the sample.  One method is called
the method of pessimistic estimators where one simply chooses the
sample incrementally according to a multiplicative weight strategy to
explicitly preserve the sizes the near linear number of cuts.\mh{this paragraph is hard to follow}

The obstruction for Li\cite{Li21} to obtaining polylogarithmic
overhead is both in the use of the expander decomposition and the fact
that even a constant factor error, much less an $n^{o(1)}$, induced by
uncrossing cuts limits the number of recursive levels to a
constant. Indeed, a recursion of depth $O(\log n)$ would be
disastrous, where fewer recursive levels are insufficient to sufficiently sparsify. \mh{it is not clear why this is the case}

We address these problems by using a modified version of techniques
from \cite{KawarabayashiT19,DBLP:journals/siamcomp/HenzingerRW20} (as
noted above) which runs faster and is better in that the uncrossing of
minimum-cuts only introduces an error of $(1+\epsilon)$ at each level
where $\epsilon = O(1/\log n)$. Thus, a subset of edges that
approximates the cuts in the resulting decomposition yields an
accurate representation of all minimum cuts.

As before, we produce these clusterings by recursively reducing the
overlap, $s$, of minimum cuts to have weight $\tilde{O}(\lambda)$. 
%As noted above, the modifications even for this are substantial. 
Producing clustering with overlap of $s$ needs modification,
as does understanding the cost of uncrossing at the detail level.  The
recursion needs significant changes due to the running time analysis
having to depend on the number of edges rather than their weight as mentioned above.  At
this point, cuts that respect the clusterings polylogarthmically
approximate minimum cuts. We then need to refine these
clusters to $(1+ O(1/\log n))$-approximate minimum cuts.

To do so, we used some new ideas which deal with a spectrum of edge
weights. We address portions of the graphs composed of small edge
weights using (modified ideas) from
\cite{KawarabayashiT19,henzinger2020local,} for simple graphs, and
address portions of the graphs with address large weight edges by
packing few trees into them.  In particular, the packing methods on
large-weight edges allow us to appropriately select small sets of
sources for the local flow procedures that find problematic
overlapping minimum cuts. We note that the localized flow methods are
similar to those used in randomized constructions of expander
decompositions \cite{DBLP:conf/soda/SaranurakW19} in addition to those
in \cite{DBLP:journals/siamcomp/HenzingerRW20}.
\mh{can you make this paragraph clearer?}


